3D Shape Generation and Completion through Point-Voxel Diffusion

We propose a novel approach for probabilistic generative modeling of 3D shapes. Unlike most existing models that learn to deterministically translate a latent vector to a shape, our model, Point-Voxel Diffusion (PVD), is a unified, probabilistic formulation for unconditional shape generation and conditional, multi-modal shape completion. PVD marries denoising diffusion models with the hybrid, point-voxel representation of 3D shapes. It can be viewed as a series of denoising steps, reversing the diffusion process from observed point cloud data to Gaussian noise, and is trained by optimizing a variational lower bound to the (conditional) likelihood function. Experiments demonstrate that PVD is capable of synthesizing high-fidelity shapes, completing partial point clouds, and generating multiple completion results from single-view depth scans of real objects.

==> figText/color.tex <==
\begin{figure}[t]
\centering
\vspace{-10pt}
\begin{tabular}{cccc}
\begin{subfigure}[b]{0.20\columnwidth}
\centering
\includegraphics[width=\linewidth]{figures/color/car1.png}
\end{subfigure}
                  &  
                  
\begin{subfigure}[b]{0.20\columnwidth}
\centering
\includegraphics[width=\linewidth]{figures/color/car1_1.png}
\end{subfigure}
                  
                  &      
\begin{subfigure}[b]{0.20\columnwidth}
\centering
\includegraphics[width=\textwidth]{figures/color/car3.png}
\end{subfigure}  &      
\begin{subfigure}[b]{0.20\columnwidth}
\centering
\includegraphics[width=\textwidth]{figures/color/car4.png}
\end{subfigure} 
\end{tabular}
\vspace{-10pt}
\caption{Colored point cloud generation trained on DensePoint cars. The left two figures show a sample car from two different views, and right two figures show two different generated cars.}
\label{fig:color}
\vspace{-10pt}
%\jw{We should show at least two views for each car, if you'd like to claim that your generation is in 3D.}
\end{figure}

